Towards Afrocentric NLP for African Languages: Where We Are and Where We Can Go

Aligning with ACL 2022 special Theme on "Language Diversity: from Low Resource to Endangered Languages", we discuss the major linguistic and sociopolitical challenges facing development of NLP technologies for African languages. Situating African languages in a typological framework, we discuss how the particulars of these languages can be harnessed. To facilitate future research, we also highlight current efforts, communities, venues, datasets, and tools. Our main objective is to motivate and advocate for an Afrocentric approach to technology development. With this in mind, we recommend \textit{what} technologies to build and \textit{how} to build, evaluate, and deploy them based on the needs of local African communities.

==> Data.tex <==
\section{Data}\label{sec:data}
A major bottleneck in the development of NLP for African languages is the paucity of machine readable data \cite{adda2016breaking} and the quality of available data. Data required for NLP should be large, and taken from an ever-growing accumulation of everyday processes in different domains of human endeavor. Without this type of data, NLP models will lack the ability to learn the implicit and explicit knowledge that is embedded in language. This is because the patterns that models need to learn can only be seen in large volumes of structured data. 

Many African languages lack the environment from which this type of machine readable data can be retrieved for many reasons. Chief among them are unfavourable language policies, socio-linguistic factors, and issues with orthography.

\subsubsection{Unfavourable Language Policies}
More than 2,000 languages have been reported in Africa - about 1/3 of all the languages in the world \cite{hammarstrom20181}, so that many African communities are multilingual. Multilingualism is not a problem in itself, but language policies in Africa treat it as such with policies that favour foreign languages or major indigenous languages to the detriment of smaller languages. In Table \ref{tab:lang-use}, we show the national\footnote{A national language is used in education, work, mass media, and government at the national level \cite{ethnologue}.}, regional\footnote{The language is used in education, work, mass media, and government within major administrative subdivisions of a nation \cite{ethnologue}.}, education\footnote{The language is in vigorous use, with standardization and literature being sustained through a widespread system of institutionally supported education \cite{ethnologue}.} languages for each county in Africa.  
%The lack of education in these languages, lack of resources for language development and lack of official status directly affect availability of machine readable data for many African languages. %Social media platforms which are often locations for crawling language specific data have few people writing completely in African languages. 

%Use the language code for the languages. Add table to the appendix
\begin{table*}[!ht]
\small
\centering
\begin{adjustbox}{max width=\textwidth}
\renewcommand{\arraystretch}{1.15}
{
        \begin{tabular}{>{}clllllll}
        \toprule

      \textbf { \small Region}    &\textbf { \small Country }   &\textbf {\small Lang(s)} & \textbf{ \small Ind.} & \textbf{ \small Nat.} & \textbf{ \small Reg.} & \textbf{ \small Edu.}\\    \toprule
      
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Burundi}} & 4 & 2 & Rundi & & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Comoros}} & 7 & 2 & French, Arabic & Comorian Ngazidja & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Djibouti}} & 5 & 2 & French, Arabic & & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Eritrea}} & 15 & 9 & Arabic & & Kunama, Tigre \\ \cline{2-8}
 \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Ethiopia}} & 91 & 87 & Amharic &Afar,Oromo, Somali, Tigrina & 31 ind and 1 foreign& \\ \cline{2-8}
 \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Kenya}} & 68 & 61 & English, Swahili & & 11 ind & \\ \cline{2-8}
 \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Madagascar}} & 14 & 12 & French, Malagasy (higher education) & &\\ \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Malawi}} & 17 & 13 & English & & Tumbuka \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Mauritius}} & 9 & 2 & English, French & & Urdu\\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Mayotte}} & 4 & 2 & French & &\\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Mozambique}} & 44 & 42 & Portuguese & & \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Reunion}} & 3 & 1 & French & &\\ \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Rwanda}} & 4 & 2 & English, French, Kinyarwanda & & \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Seychelles}} & 3 & 1 & English, French, Creole & & \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Somalia}} & 13 & 10 & Arabic, Somali & & English \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{}} &&  &  &Sudanese Arabic, Bari, &  \\ 
   \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{South Sudan}} & 70 & 59 & English &Juba Arabic, Zande & 8 ind.  \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Tanzania}} & 126 & 118 & Swahili & & English and Swahili\\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Uganda}} & 44 & 41 & English, Swahili & & 2 ind. , 1 non-ind..  \\ 
 \cline{2-8}
  \multicolumn{1}{c}{}  &   \multirow{1}{*}{\textbf{Zambia}} & 46 & 37 & English & 3 indigenous languages & 4 ind., 1 non-ind.\\ 
 \cline{2-8}
 \multicolumn{1}{c}{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{\small East Africa}}}}  &  Zimbabwe & 22 & 16 & English & & 2 ind, 2 south African languages\\ 
\cline{2-8}
    \toprule 
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Angola}} & 46 & 41 & Portuguese & &\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Cameroon}} & 275 & 271 & English, French & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Central African Republic}} & 75 & 65 & English, Sango & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Chad}} & 129 & 123 & French, Arabic & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Congo}} & 66 & 55 & French & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Democratic Republic of Congo}} & 214 & 209 & French & & 2 ind.\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Equatorial Guinea}} & 15 & 12 & Spanish & & 2 foreign  \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Gabon}} & 43 & 40 & French & & \\ \cline{2-8}
 \multicolumn{1}{c}{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{ \small Middle Africa}}}}  &Sao Tome e Principe  & 7 & 3 & Portuguese & & 1 foreign \\ \cline{2-8}
    \toprule 
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Algeria}} & 19 & 14 & Arabic, Amazigh & & 1 foreign \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Egypt}} & 19 & 9 & Arabic & &  \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Libya}   } & 9 & 8 & Arabic & &  \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Morocco}   } & 15 & 10 & Arabic Tamazight & &  \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Sudan}   } & 75 & 70 & Arabic, English & & \\ \cline{2-8}
 \multicolumn{1}{c}{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{North Africa}}}}  & Western Sahara & 4 & 2 & Arabic & & \\ \cline{2-8}
    \toprule 
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Botswana}} & 31 & 26 & English and Setswana & & 1 foreign \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Eswatini}} & 5 & 1 & English, Swari & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Lesotho}} & 5 & 3 & English and Sotho & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Namibia}} & 28 & 23 & English & & 3 foreign, 6 ind.\\ 
\cline{2-8}
{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{\small South Africa}}}}  & & & & English, Afrikaans, Ndebele, Setswana, \\
{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{\small }}}}  & & & &  North Sotho, South Sotho, Swati,  \\
{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{}}}} & \texbf{\small South Africa} & 31 & 20 &  Tsonga, Venda, Xhosa, Zulu & & 1 foreign 
\\ 
\cline{2-8}
    \toprule 
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Benin}} & 55 & 50 & French & &\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Burkina Faso}} & 71 & 66 & French && \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Cape Verde Islands}} & 2 & 1 & Kabyverdianu, Portuguese & &  \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Cote d'ivoire}} & 87 & 75 & French & & 1 foreign\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Gambia}} & 11 & 7 & English & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Ghana}} & 83 & 73 & English & Farefare, Mampruli & 5 ind\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Guinea}} & 37 & 35 & French & Pular & 3 ind\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Guinea-Bissau}} & 23 & 18 & Portuguese & &\\ \cline{2-8}
\multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Liberia}} & 31 & 27 & English & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Mali}} & 68 & 63 & French  & & 5 ind., 1 foreign\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Mauritania}} & 7 & 5 & Arabic & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Niger}} & 23 & 19 & French & & 2 ind., 1 foreign \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Nigeria}} & 522 & 512 & English & Hausa, Igbo, Yor\`{u}b\'{a} & 5 ind.\\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Saint Helena}} & 1 & 0 & English && \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Senegal}} & 39 & 31 & French & & \\ \cline{2-8}
 \multicolumn{1}{c}{}  & \multirow{1}{*}{\textbf{Sierra Leone}} & 24 & 19 & English & Limba, Mende, Themne & \\ \cline{2-8}
 \multicolumn{1}{c}{\multirow{-6}{*}{\rotatebox[origin=c]{90}{\textbf{\small West Africa}}}}  & Togo & 44 & 40 & French & & \\ \cline{2-8}
    \toprule 
\end{tabular}}
\end{adjustbox}
\caption{A statistics of the language use in Africa computed from \cite{ethnologue}. For each country, we show the number of languages (lang) reported, the number of indigenous languages spoken in the country (ind), the national language (nat.), the regional languages (reg) and the educational languages (edu).  }\label{tab:lang-use}
\end{table*}

\note[mam]{This situation involves Indigenous languages. For example, ...}

Out of the 54 countries in Africa, only 17 countries have an indigenous language as a national language although in most cases, a foreign language is the main official language. Furthermore, the countries that give any official status to indigenous language use the indigenous languages with majority speakers. In Nigeria, 3 out of 512 languages are officially recognized as regional languages; Ghana uses 13 of its 73 indigenous languages as institutional languages; Swahili is the only official indigenous language in Tanzania out of 118 others; 12 of 61 languages in Kenya have some official status, while 12 of 20 indigenous languages in South Africa are institutional languages. 

\note[mam]{These unfavorable policies directly negatively impact data availability, etc. }

Since these "minor" languages do not often have official status, they are not used in education, do not have orthographies, or exist in print only as bibles. This results in the diminishing use of smaller African languages. Small African languages are further weakened when speakers of these languages need to learn the major languages in other to communicate in the larger society. The minority languages in Tanzania for instance are "only spoken in the home, and they are severely threatened by Swahili. In public areas, the minority languages are not at all heard; their usage is prohibited in education, and discouraged at political gatherings and religious meetings; they are not used by any radio or television station; and there are no newspapers published in any of them" \cite{petzell2012linguistic}. In Nigeria, most of the few resources available for language development is poured into the 3 regional languages: Yor\`{u}b\'{a}, Igbo and Hausa with little left for non-regional languages. It is important to mention that some of these non-regional languages may have millions of L1 speakers. 

In countries where an indigenous language has official or regional status, adequate resources may not be available for the implementation of such policies. In Nigeria for instance, although the national policy of education requires that the language of the immediate community or the regional language be used as the medium of instruction in early education, lack of adequate educational resources in indigenous languages, and teachers trained to teach in indigenous languages makes the policy difficult to implement. In fact in recent amendments to the policy, specific mention of the three regional language have been removed indicating the lack of commitment necessary to develop these languages \cite{trudell2018language}. In many schools indigenous languages are referred to as vernaculars and are prohibited. Violation usually attracts fines and many times corporal punishment. 

Lack of official status of many African language leads to lack of education and resources for language development, So we include in our concept of a grand challenge the need to develop language policies that favour the use of African languages for use in everyday transactions. Favourable language policies will significantly transform NLP of African languages.

% Create a map for pidgins in Africa, creaoles. 

%In the north of Nigeria where Hausa is the regional language, speakers of smaller languages speak Hausa thus reducing the use of their own indigenous languages.

%In addition, many of the countries with a language policy that offers official or national language status to some indigenous languages only pay lip service to these policies. Nowhere in Africa is this more evident than in the Nigeria \cite{trudell2018language}. Nigeria has 512 indigenous languages, indeed the highest in any African country \cite{ethnologue}. Out of the 512 indigenous languages in Nigeria, three languages were selected as regional languages. The regional languages: Yor\`{u}b\'{a} in the west with about 40 million L1 speakers, Igbo in the east with about 29 million L1 speakers and Hausa in the north with approximately 36 million L1 speakers are in turn dominated by English and are described as deprived languages \cite{bamgbose1993deprived}. 


\subsubsection{Socio-linguistic Factors}
One of the relics of colonization in Africa is the preference for and prolific use of foreign languages. This is evident in the language attitudes and choices of many Africans. Colonialism imported English, French and a few other foreign languages to Africa and some foreign languages have since been adopted as the official language in government, education and most official businesses in many African countries. 46 countries use one of English, French, Spanish or Portuguese for some official business. 

In Nigeria, English is the language of the elite, and fluency in English is synonymous with a good education \cite{trudell2018language}. The desire for fluency in English is legitimised by the Nigerian job market that rewards fluency in English. Fluent speakers of English earn more than their non-fluent or non-English speaking counterparts \cite{pinon2010english}. As a result, many parents, even those who can barely speak English prefer and ensure that their children are taught in English right from the elementary classes. Bilingualism is also believed to affect children's ability to attain competence in English and thus parents avoid speaking mother tongues at home for fear of raising children with poor communication in English. Many children in urban areas therefore can neither speak, read, nor write in indigenous languages and many do not even understand the languages at all.

%by Nigerian citizens and government today \cite{trudell2018language}. 
In Tanzania, although Kiswahili is the official language, Kiswahili is associated with traditional values while English is used in government administration, the High court, diplomacy, education, and foreign trade \cite{petzell2012linguistic, mohr2018changing}. English is seen as a prerequisite for scientific and technological development and a key to social prestige and power. Although primary education in Tanzania is in one of English or Swahili \cite{foster2021language}, according to \cite{petzell2012linguistic}, a student who succeeds in all schools subjects apart from English cannot continue studying at higher levels. English is introduced as a subject in the third year of primary school and it becomes the medium of instruction in the first year of secondary school. Swahili is offered as a subject throughout school and university, but the medium of instruction at all levels above primary school is English. Tanzanians like Nigerians thus seek competence in English as a status symbol, and to obtain well paying jobs \cite{mohr2018changing}

The linguistic attitudes of Nigerians and Tanzanians which is representative of many Africans therefore has significant impact on the availability of digital language resources for NLP in Africa. A change in language preference therefore can only be achieved through consistent decolonization of African people. So we include in our concept of a grand challenge the need for Africans to see their language as good and not inferior to colonial languages. 

%have thus affected the economic values of African languages and . The vast majority of people who can afford technology that can drive language development for natural language processing are not 

\subsubsection{Issues with orthography}\label{subsubsection:ortho}
Many African languages are written with latin scripts and diacritics to represent tone, length, and other grammatical features. However, many African languages do not have language-specific keyboards, which makes it difficult writing African languages correctly on a computer or smart phone. This is worsened by the relatively poor or non-existent education in African languages that negatively affects the proficiency of native speakers in writing their own language. For these reasons, those who write African languages may inconsistently omit tones and other diacritics that would significantly reduce ambiguity in written documents. Some writers can use conventional keyboards to write but some other do not know how to use conventional keyboards or do not know the correct diacritics.  

%Proficient users of African languages who can be assumed to be in the minority are able to use diacritics in digital text however, since many others cannot written documents are inconsistently marked.
The inconsistencies introduced into written documents affect results of search engines \cite{choros2005testing}. Search engines do not recognize the relationship between diacritized text and its undiacritized counterparts\cite{asubiaro2014effects} and it results in difficulty in retrieving resources for many African languages. To optimize searches for African languages with diacritics therefore, some writers use normalized text. This results in a mismatch between the writing for documents on the web and standard writing variety of African languages in other sources like books. 

Furthermore, orthographies for many languages may not be standardized. Word boundaries may not be standardized, spellings can vary, and even the usage of the language itself may not be consistent from speaker to speaker. While many languages do have some sort of dictionary or word list, many of these resources were created by foreign linguists and don’t necessarily represent a standardized spelling. Languages that have standard orthographies still suffer from these inconsistencies as standard spelling conventions are not followed resulting in lack of uniformity in spellings and punctuation and a chaotic writing system \cite{olumuyiwa2013yoruba}.

A third problem is that while dialects and their relationships to one another are well understood for the world’s most prominent languages, they are often quite unclear when dealing with less studied languages. Mutual intelligibility is often used as a measuring stick for determining the relationship of two languages (whether separate languages or merely separate dialects), but this measure can be somewhat subjective. As a result, it is not uncommon to find that two different sources of text presented as belonging to the same language can exhibit substantial differences, leading to questions for NLP researchers of whether their tools are even applicable to the presented texts.

Multilingualism, socio-linguistic factors, and issues with orthography all contribute to low availability, discoverability, reproducibility, focus and lack of benchmarks \cite{martinus2019focus} for many African languages.
%Diacritics are usually adopted to represent tone, and other linguistic information. 
%However, the proliferation of the internet in urban areas of Africa, has provided more accessibility to language data over the internet. This enables the collection of large corpora through crawling the web,  although this type of data cannot be guaranteed to be clean or consistency. 

%In addition, since many African languages are tone marked using diacritic marks, many data sources omit the diacritics resulting in many ambiguities introduced to the data for many languages.

%\section{Some ongoing interesting NLP projects}
%\begin{itemize}
%    \item \url{https://kamusi.org/}
%    \item \url{https://brandeis.app.box.com/s/nigx0bt0ayx25zp0hik36t681grpyqwr}
%    \item \url{https://github.com/allenai/allennlp/discussions/5265}
%    \item \url{https://github.com/Andrews2017/africanlp-public-datasets}
%    \item \url{https://paperswithcode.com/dataset/common-voice}
%    \item \url{https://docs.google.com/spreadsheets/d/1p_HpKkrAlRDte04pgStsxaN8IJ4I0GgidVGIE_6VtMw/edit#gid=2144185743}
%    \item \url{https://www.k4all.org/project/}
%\end{itemize}

%\section{Data Collection process}
%Data collection is often by crawling the world wide web \cite{}. Collection is often done by novices, not much work is done on human evaluation

\subsection{Data Quality}
A manual evaluation of 205 corpora for African NLP including CCAligned \cite{elkishky_ccaligned_2020}, ParaCrawl \cite{banon-etal-2020-paracrawl, espla2019paracrawl}, WikiMatrix \cite{schwenk2019wikimatrix}, OSCAR \cite{suarez2020monolingual}, and mC4 \cite{xue-etal-2021-mt5} showed that at least 15 corpora were completely erroneous, a significant fraction contained less than 50\% of correct data, and 82 corpora were mislabelled or used ambiguous language codes \cite{caswell2021quality}. The inaccuracy is due to a lack of or poor quality of (1) language identification tools, (2) dictionaries, (3) text preprocessing piplelines to name a few that are required to build high quality datasets. Furthermore, available resources are rarely evaluated especially when crawled as part of a multilingual dataset. The poor data quality consequently affects downstream models. ~\newcite{alabi2020massive} find that for instance, the fastText embeddings for Yor\`{u}b\'{a} has an estimated 135k out of 150K words belonging to other languages such as English, French, and Arabic. Models trained on a cleaned corpus that they created outperformed models trained with the off-the-shelf fasttext embeddings even though their embedding had fewer words. 

Due to issues to orthography discussed in {subsubsection:ortho}, several discrepancies occur with the language use on the web and those in physical books for many African languages. For languages with tone, whereas tone is often represented in books, it is not uncommon for media sources from which many NLP data are crawled to omit tones diacritics in written documents. All VOA websites, for instance omit tone for African languages with tone diacritics. BBC omits tone for all Yor\`{u}b\'{a} texts except the headlines, JW300 also omits tone for many African languages. This introduces a higher level of ambiguity which even human experts find challenging to unravel. 
%a lack of evaluation of large data crawled from the web and 

%They also collect high quality and noisy data for the two languages and quantify the improvements that depend not only on the amount of data but on the quality too. They also use different architectures that learn word representations both from surface forms and characters to further exploit all the available information which showed to be important for these languages. For the evaluation, they manually translate the wordsim-353 word pairs dataset from English into Yor\`{u}b\'{a} and Twi. They extend the analysis to contextual word embeddings and evaluate multilingual BERT on a named entity recognition task. For this, they annotate with named entities the Global Voices corpus for Yor\`{u}b\'{a}. They found that noise adversely affected the correlation with human judgments even though they used more data. For noise they introduced words without diacritics which increased the ambiguity of the words. Their contribution is the output of the work, corpora provided, embeddings and the test suits for both languages. 

\subsection{Foreign terminologies}
Although a form of code mixing, this is slightly different in that there are no words for certain terms in many African languages and foreign words are borrowed to express those terms in African languages. This is partly due to the lack of constant usage of African languages in contexts such as governance, law, technology, science, education to name a few which in turn prevents African languages from expanding in vocabulary to accommodate concepts that have become important topics for conversation. Available data for many African languages are also translations of English or French and do not essentially reflect the language usage of the people. This results in borrowed words in the documents due to the absence of those concepts in the target African language. 

Furthermore, terminologies are used inconsistently and spelt differently by the same people. Jehovah's witness data for instance has \texttt{Jehovah} as its most frequent words. Many African languages data thus show an overdependence on loan words which are not even made to conform to the phonological structure of the African languages. An evaluation of some datasets found at least 5\% of words used in the are loan words and 95\% of those loan words do not conform to the phonology of the African language. 

This is problematic because users of the language do not know these foreign terminologies. Literacy is low. Data used for NLP is known to be biased in the best case scenarios, but in the worst case just like this, it is problematic.

%Evaluation of loan words in Akan, Swahili, Yoruba

%Many African languages have a low status in their communities resulting in less development. Languages grow and evolve with use. It grows with that which it is fed. Language of interaction matters. If African languages are used to interact with technology, terminology will grow significantly. 

\subsection{Errors in text due to a lack of spelling checkers}
Many African languages lack spelling checkers and many datasets do not go through any form of editing. Failure to evaluate datasets is partly due to the lack of available resources including dictionaries, grammar books, or primers for many African languages. According to \cite{hock2011world}, grammatical information is lacking for almost half of Africa’s languages leaving Africa the second least known continent (after Oceania, dominated by the New Guinea area). To manually edit data with several thousands or millions of words therefore may be unrealistic for many languages without spelling checkers. This has resulted in a blind spot created by research that aims only to improve accuracy on available datasets and does not investigate the representativeness or quality of the data, or the ways in which different errors have different human values and consequences. A single error in diacritic assignment for instance can result in significant semantic and syntactic differences in texts and this leaves much to be considered when we realize that texts are often neither manually nor automatically evaluated. 

Furthermore, a huge portion of the languages that have dictionaries or other grammar books adopt a different convention from those used for many NLP texts. Inconsistent orthographies often radically differ from real world data and standard orthographies. Therefore, as soon as these technologies are applied to the real world data, performance drops. Using Hausa as an example, different dictionaries adopt different conventions \cite{schuh_yalwa_1993}. Hausa is written with Ajami scripts or Romanized scripts. All commercially published books and nearly all Hausa language newspapers use the Romanized orthography while poetic literature and some spiritual texts use the Ajami orthography. Standard Romanized orthography is written without tones or any indication of vowel length. The orthography used in grammars, dictionaries, and pedagogical documents on the other hand, indicate tone and vowel length. These result in significant spelling, punctuation, and stylistic differences that may make developing generalizable spelling checkers a little more challenging. This problem may be worsened in scenarios where standard and non-standard conventions are adopted in the same text without prior information of the writing convention adopted. 

The implication of inconsistencies in orthography is enormous for low resource languages. First is the problem of data sparsity which is heightened when different spellings of the same word are used in the same text, or when tone or other grammatical features are inconsistently marked. Training with data from different domains may also not yield the same dividends as in languages where orthographies are used more consistently. Furthermore, domain adaptation which is based on the unrealistic assumption that the target domain is known may not apply consistently for most African languages. The reliability of the models trained with erroneous data is also somewhat lower than those trained with cleaned data. 

\subsection{Language change over time}
Language data for African languages is not available at the rate at which language change occurs overtime. Variation in language is ubiquitous, particularly in newer forms of writing such as social media. This results in a mismatch between language use in society and data available in digital formats. Orthography standards, phonological patterns, semantics, syntax, and every aspect of language changes over time. This is especially true for labelled data because annotation requires time. At the same time, ways
of communication change, so what we annotate today might be very distant to what we need to process tomorrow. Moreover, it might not be trivial to find the right annotators; annotation schemes might need adaptation as well and tradeoffs for doing so need to be defined \cite{plank2016non}.

Without quality data, growth of language terminologies, and the development of generalizable spelling checkers in African languages, many errors in documents in addition to inconsistencies aforementioned will not be noticed. So we include in our concept of a grand challenge the open research questions that should inspire more attention to data used for NLP of African languages.


\begin{table*}[!ht] %Use language codes 

%An annoymous repository to go with the submission. 

\centering
\begin{adjustbox}{max width=\textwidth}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{p{3cm}p{3cm} p{3cm}p{3cm}} 
\hline
\thead{\textbf{Language }} & \thead{\textbf{Language code}} & \thead{\textbf{Language }} & \thead{\textbf{Language code}} \\ \hline  \hline
Rundi & run & Kabiye & kab \\ \hline
French & fra & Kongo & kon\\ \hline
Arabic & ara & Kikuyu & kik\\ \hline 
Comorian Ngazidja & zdj & Kuanyama & kua \\ \hline 
Kunama & kun  & Kanuri & kau \\ \hline 
Tigre & tig & Lingala & lin  \\ \hline
Amharic & amh & Ndonga & ndo\\ \hline
Afar & aar & Tigrinya & tir\\ \hline
Oromo & gaz & Wolayatta & wal\\ \hline
Somali & som & Ge'ez & gez \\ \hline
Fulah & ful  & Kamba & kam \\ \hline
English & eng & Nyanja & nyj  \\ \hline
Swahili & swa  & Efik & efi \\ \hline
Malagasy & mlg & Edo & bin\\ \hline
Tumbuka & tum & Dendi & ddn\\ \hline
Urdu & urd & Fon & fon\\ \hline
Portuguese & por  & Esan & ish \\ \hline
Kinyarwanda & kin & Isoko & iso\\ \hline
Seychelles French Creole & crs  & Kimbudu & kmb \\ \hline
Arabic Sudanese Spoken & apd  & Tshiluba & lua\\\hline
Bari & bfa & Tiv & tiv \\\hline
Juba Arabic & pga & Urhobo & urh\\\hline
Zande & zne & Swahili Congo & swc \\\hline
Sango & sag & Bemba & bem \\\hline
Spanish & spa & Dinka & din\\\hline
Amazigh & kab & Lukpa & dop \\\hline
Tamazight & tzm & Tachelhit & shi\\\hline
Setswana & tsn & Tamajaq & ttq\\\hline
Swati & ssw & Zama & xuu \\\hline
Southern Sotho / sesotho & sot  & Mboshi & mdw \\\hline
Afrikaans & afr & coastal Swahili & swa \\\hline
Ndebele & nbl & \'{E}w\'{e} & ewe\\\hline
Setswana & tsn & Bambara & bam \\\hline
Northern Sotho /Sepedi & nso & Twi / Akan & aka  \\\hline
Tsonga & tso & Nigerian Pidgin & pcm \\\hline
Venda / Tshivenda & ven  & Luo & luo \\\hline
Xhosa & xho & Wolof & wol\\\hline
Zulu & zul & Luganda & lug \\\hline
Kabyverdianu & kea & Chichewa / Cinyanja& nya\\ \hline
Farefare & gur & Shona & sna  \\ \hline
Mampruli & maw & Themne & tem\\ \hline
Pular & fuf & Mende & men\\ \hline
Hausa & hau & Limba & lma\\ \hline
Igbo & ibo & Limba & lma \\ \hline
Yor\`{u}b\'{a} & yor && \\ \hline


 \end{tabular}
 \end{adjustbox}
 \caption{The language codes for all languages referenced in this paper} \label{tab:resources}
 \end{table*}

==> data-availability.tex <==
\section{Data Practices and Discoverability}\label{sec:data-availability}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Unlike other digitally transformed societies that have mature language policies and standardized orthographies, the data situation in Africa is quite challenging. While, for example, social media is a venue for data collection for many high-resource languages, most Africans post in foreign languages rather than in Indigenous languages~\cite{malatji_2019}.\footnote{https://www.talkwalker.com/quick-search.} One reason behind this issue is unavailability of keyboards for Indigenous languages. For example, most keyboards do not support diacritics for representing tone \textcolor{red}{or other grammatical features}. Partial or complete lack of writing literacy is another reason. A third reason is related to access to smart machines and internet connectivity. Collectively, these compounded issues mean there are only few (and often smaller) online communities that contribute to web fora, Wikipedias, and other platforms where data is growing in large-to-massive amounts for high-resource languages. 

%access to stable orthographic practices also contributes to the paucity of online data. Many African languages are written with latin scripts, and diacritics to represent tone, length, and other grammatical features. However, many African languages do not have language-specific keyboards, which makes it difficult writing African languages correctly on a computer or smart phone. This is worsened by the relatively poor or non-existent education in African languages that negatively affects the proficiency of native speakers in writing their own language \cite{cahill2001avoiding}. For these reasons, those who write African languages may inconsistently omit tones and other diacritics that would significantly reduce ambiguity in written documents. 

%In domains like social media, where African can freely choose their preferred language, Africans have shown preference for foreign languages with many African languages absent in cyberspace because Africans are reluctant to use their languages online and not literate enough to write in their native languages. There is even a dearth of research in this area. Analysis of social media platforms in Africa showed a paucity of indigenous language usage. In South Africa for instance, social media platforms like Facebook, Instagram, Twitter, and Tiktok are dominated by English~\cite{malatji_2019} with about 91\% of conversations being in English.\footnote{https://www.talkwalker.com/quick-search}

%Colonialism imported English, French, Portuguese, and foreign languages have been viewed as a symbol of status, class, or literacy. In Nigeria, English is the language of the elite, and fluency in English is synonymous with a good education \cite{trudell2018language}. The desire for fluency in English is legitimised by the Nigerian job market that rewards fluency in English. Fluent speakers of English earn more than their non-fluent or non-English speaking counterparts \cite{pinon2010english}. As a result, many parents, even those who can barely speak English prefer and ensure that their children are taught in English right from the elementary classes. Bilingualism is also believed to affect children's ability to attain competence in English and thus parents avoid speaking mother tongues at home for fear of raising children with poor communication in English. Many children in urban areas therefore can neither speak, read, nor write in indigenous languages and many do not even understand the languages at all.

%by Nigerian citizens and government today \cite{trudell2018language}. 
%In Tanzania, although Kiswahili is the official language, Kiswahili is associated with traditional values while English is used in government administration, the High court, diplomacy, education, and foreign trade \cite{petzell2012linguistic, mohr2018changing}. English is seen as a prerequisite for scientific and technological development and a key to social prestige and power. Although primary education in Tanzania is in one of English or Swahili \cite{foster2021language}, according to \cite{petzell2012linguistic}, a student who succeeds in all schools subjects apart from English cannot continue studying at higher levels. English is introduced as a subject in the third year of primary school and it becomes the medium of instruction in the first year of secondary school. Swahili is offered as a subject throughout school and university, but the medium of instruction at all levels above primary school is English. Tanzanians like Nigerians thus seek competence in English as a status symbol, and to obtain well paying jobs \cite{mohr2018changing}.


% Some writers can use conventional keyboards to write but some other do not know how to use conventional keyboards or do not know the correct diacritics.  

%Proficient users of African languages who can be assumed to be in the minority are able to use diacritics in digital text however, since many others cannot written documents are inconsistently marked.

Data discoverability is another important issue. One problem contributing to poor discoverability \cite{martinus2019focus} of online data for African languages is orthographic inconsistencies. In many cases, as implied earlier, orthographies may not be standardized. There is also significant spelling variation. While some languages do have some sort of a dictionary or a word list, the majority of these resources do not necessarily represent a standardized spelling. Languages that have standard orthographies also suffer from these inconsistencies as standard spelling conventions are not followed resulting in lack of uniformity in spellings and punctuation, amounting to `chaotic' writing systems~\cite{olumuyiwa2013yoruba}. Orthographic inconsistencies affect results of search engines~\cite{choros2005testing} in that these engines do not recognize the relationship between diacritized text and its undiacritized counterparts~\cite{asubiaro2014effects, olumuyiwa2013yoruba}. This results in difficulty retrieving resources for many African languages. To optimize search for African languages that involve diacritics, some users employ normalized text. This in turn creates a mismatch between web documents and other standard offline documents such as books for many African languages.

Furthermore, inconsistent orthographies often radically differ from real world data and standard orthographies. Therefore, as soon as these technologies are applied to the real world data, performance will drop. Using Hausa as an example, all commercially published books and nearly all Hausa language newspapers use the romanized orthography. Standard romanized orthography is written without tones or any indication of vowel length~\cite{schuh_yalwa_1993}. The orthography used in grammars, dictionaries, and pedagogical documents on the other hand, indicate tone and vowel length~\cite{schuh_yalwa_1993}. In addition, methods and practices for content archiving also favour foreign languages. For example, all VOA websites, omit tone for African languages with tone diacritics. BBC also omits tone for all Yor\`{u}b\'{a} texts except the headlines, JW.org also omits tone for many African languages. %These introduce a higher level of ambiguity which even human experts find challenging to unravel with significant spelling, punctuation, and stylistic differences. This problem may be worsened in scenarios where standard and non-standard conventions are adopted in the same text without prior information of the writing convention adopted. 

\textbf{Recommendations.} \textbf{(1)} We recommend the development of keyboards that accommodate African languages. \textbf{(2)} We also suggest orchestrated efforts within the different communities to standardize writing for the various languages. \textbf{(3)} Awareness about development of policies around data collection that respect user privacy and data sovereignty will also benefit African communities. \textbf{(4)} Search engines can also help Africans by developing algorithms that facilitate data discoverability so that Africans can search in their own Indigenous languages. We now discuss data quality. 

%\language specific keyboards to aid the use of African languages online.  These will render tremendous service to the availability of big data that truly represent the context of use of these languages. 

%A third problem is that while dialects and their relationships to one another are well understood for the world’s most prominent languages, they are often quite unclear when dealing with less studied languages. Mutual intelligibility is often used as a measuring stick for determining the relationship of two languages (whether separate languages or merely separate dialects), but this measure can be somewhat subjective. As a result, it is not uncommon to find that two different sources of text presented as belonging to the same language can exhibit substantial differences, leading to questions for NLP researchers of whether their tools are even applicable to the presented texts. Nigerians, Tanzanians, and South

%The lack of documentation in indigenous languages, linguistic attitudes of Africans, and the challenges with orthography all contribute to low availability, discoverability, reproducibility, focus, and lack of benchmarks \cite{martinus2019focus} for many African languages.

%A change in language preference therefore can only be achieved through consistent decolonization of African people. So we include in our concept of a grand challenge the need for Africans to see their language as good and not inferior to colonial languages. 


%Policies that govern language use, the language preferences of the African people, and literacy in African languages contribute significantly to the paucity of machine readable data of many African languages. 

%Language policies contributes significantly here. With most African languages lacking official statuses in the domain in which they are spoken, (details in Section \ref{sec:f_engineering}

%Chief among them are unfavourable language policies, socio-linguistic factors, and issues with orthography.

%\subsubsection{Unfavourable Language Policies}
%More than 2,000 languages have been reported in Africa - about 1/3 of all the languages in the world (that is 54 of 196 countries in the word) \cite{hammarstrom20181, ethnologue}. 

%The language policies in most African countries favour foreign languages or major indigenous languages to the detriment of smaller languages. In Table \ref{tab:lang-use}, we show the national\footnote{A national language is used in education, work, mass media, and government at the national level \cite{ethnologue}.}, regional\footnote{The language is used in education, work, mass media, and government within major administrative subdivisions of a nation \cite{ethnologue}.}, education\footnote{The language is in vigorous use, with standardization and literature being sustained through a widespread system of institutionally supported education \cite{ethnologue}.} languages for each county in Africa.  


%\note[mam]{This situation involves Indigenous languages. For example, ...}

%As seen in Table \ref{tab:lang-use}, out of the 56 countries in Africa, only 17 countries have an indigenous language as a national language, although in 14 of these 17 countries, a foreign language is the main official language. Furthermore, the countries that give any official status to indigenous language use the indigenous languages with majority speakers. In Nigeria, 3 out of 512 languages are officially recognized as regional languages; Ghana uses 13 of its 73 indigenous languages as institutional languages; Swahili is the only official indigenous language in Tanzania out of 118 others; 12 of 61 languages in Kenya have some official status, while 12 of 20 indigenous languages in South Africa are institutional languages. 

%These unfavorable policies have a direct negative impact on data availability. First, most African languages (those without any official status) are used only at home. The minority languages in Tanzania for instance are "only spoken in the home. In public areas, the minority languages are not at all heard; their usage is prohibited in education, and discouraged at political gatherings and religious meetings; they are not used by any radio or television station; and there are no newspapers published in any of them" \cite{petzell2012linguistic}. In Nigeria, most of the few resources available for language development is poured into the 3 regional languages: Yor\`{u}b\'{a}, Igbo, and Hausa with little left for non-regional languages. It is important to mention that some of these non-regional languages may have millions of L1 speakers. This results in the diminishing use of most African languages and consequent unavailability of data in domains such as education, government, politics, news, to name a few in most languages. 

%in education, do not have orthographies, or exist in print only as bibles - therefore data related to most domains of human existence are not available. Many African languages are further weakened when native speakers need to learn the foreign or major languages in other to communicate in the larger society. 

%In countries where an indigenous language has official status, governments and implementing bodies only pay lip service to these policies that exist only in paper \cite{ThePoliticsofLanguageEducationinAfrica}. In Nigeria and Senegal for instance, although their language policies recommend that some indigenous languages be used in education, the national assembly, and other domains, lack of trained personnel, adequate educational resources in indigenous languages, and teachers trained to teach in indigenous languages, makes the policy difficult to implement. In fact in recent amendments to the policy in Nigeria, specific mention of the three regional language have been removed indicating the lack of commitment necessary to develop these languages \cite{trudell2018language}. In Senegal on the other hand, no indigenous language is used in any official domain \cite{ThePoliticsofLanguageEducationinAfrica}. The result is the absence of data in indigenous languages in any of these official domains. 

%\subsubsection{Socio-linguistic Factors}
%One of the relics of colonization in Africa is the preference for and prolific use of foreign languages. This is evident in the language attitudes and choices of many Africans. Colonialism imported English, French, and a few other foreign languages to Africa and some foreign languages have since been adopted as the official language in government, education and most official businesses in many African countries \cite{ThePoliticsofLanguageEducationinAfrica}. 46 countries use one of English, French, Spanish or Portuguese for some official business \cite{ethnologue}. 

%In Nigeria, English is the language of the elite, and fluency in English is synonymous with a good education \cite{trudell2018language}. The desire for fluency in English is legitimised by the Nigerian job market that rewards fluency in English. Fluent speakers of English earn more than their non-fluent or non-English speaking counterparts \cite{pinon2010english}. As a result, many parents, even those who can barely speak English prefer and ensure that their children are taught in English right from the elementary classes. Bilingualism is also believed to affect children's ability to attain competence in English and thus parents avoid speaking mother tongues at home for fear of raising children with poor communication in English. Many children in urban areas therefore can neither speak, read, nor write in indigenous languages and many do not even understand the languages at all.

%by Nigerian citizens and government today \cite{trudell2018language}. 
%In Tanzania, although Kiswahili is the official language, Kiswahili is associated with traditional values while English is used in government administration, the High court, diplomacy, education, and foreign trade \cite{petzell2012linguistic, mohr2018changing}. English is seen as a prerequisite for scientific and technological development and a key to social prestige and power. Although primary education in Tanzania is in one of English or Swahili \cite{foster2021language}, according to \cite{petzell2012linguistic}, a student who succeeds in all schools subjects apart from English cannot continue studying at higher levels. English is introduced as a subject in the third year of primary school and it becomes the medium of instruction in the first year of secondary school. Swahili is offered as a subject throughout school and university, but the medium of instruction at all levels above primary school is English. Tanzanians like Nigerians thus seek competence in English as a status symbol, and to obtain well paying jobs \cite{mohr2018changing}

%The linguistic attitudes of Nigerians and Tanzanians which is representative of many Africans therefore has significant impact on the availability of digital language resources for NLP in Africa in many domains.

%\subsubsection{Issues with orthography}\label{subsubsection:ortho}
%Many African languages are written with latin scripts, and diacritics to represent tone, length, and other grammatical features. However, many African languages do not have language-specific keyboards, which makes it difficult writing African languages correctly on a computer or smart phone. This is worsened by the relatively poor or non-existent education in African languages that negatively affects the proficiency of native speakers in writing their own language. For these reasons, those who write African languages may inconsistently omit tones and other diacritics that would significantly reduce ambiguity in written documents. Some writers can use conventional keyboards to write but some other do not know how to use conventional keyboards or do not know the correct diacritics.  

%Proficient users of African languages who can be assumed to be in the minority are able to use diacritics in digital text however, since many others cannot written documents are inconsistently marked.
%The inconsistencies introduced into written documents affect results of search engines \cite{choros2005testing}. Search engines do not recognize the relationship between diacritized text and its undiacritized counterparts\cite{asubiaro2014effects} and it results in difficulty in retrieving resources for many African languages. To optimize searches for African languages with diacritics therefore, some writers use normalized text. This results in a mismatch between the writing for documents on the web and standard writing variety of African languages in other sources like books. 

%Furthermore, orthographies for many languages may not be standardized. Word boundaries may not be standardized, spellings can vary, and even the usage of the language itself may not be consistent from speaker to speaker. While many languages do have some sort of dictionary or word list, many of these resources were created by foreign linguists and don’t necessarily represent a standardized spelling. Languages that have standard orthographies still suffer from these inconsistencies as standard spelling conventions are not followed resulting in lack of uniformity in spellings and punctuation and a chaotic writing system \cite{olumuyiwa2013yoruba}.

%A third problem is that while dialects and their relationships to one another are well understood for the world’s most prominent languages, they are often quite unclear when dealing with less studied languages. Mutual intelligibility is often used as a measuring stick for determining the relationship of two languages (whether separate languages or merely separate dialects), but this measure can be somewhat subjective. As a result, it is not uncommon to find that two different sources of text presented as belonging to the same language can exhibit substantial differences, leading to questions for NLP researchers of whether their tools are even applicable to the presented texts.


%\subsection{Recommendations}
%Unfavourable language policies, socio-linguistic factors, and issues with orthography all contribute to low availability, discoverability, reproducibility, focus and lack of benchmarks \cite{martinus2019focus} for many African languages. We thus make the following recommendations:

%\begin{enumerate}
%    \item Lack of official status of many African language leads to lack of education and resources for language development. So, we include in our concept of a grand challenge, the need to develop language policies that favour the use of African languages for use in everyday transactions. Favourable language policies will significantly increase the availability of data for African languages.
%    \item A change in language preference therefore can only be achieved through consistent decolonization of African people. So we include in our concept of a grand challenge the need for Africans to see their language as good and not inferior to colonial languages. 
%    \item 
%\end{enumerate}


%Creoles and pidgin. 

%Limitations in existing work and opportunities


==> introduction.tex <==
\section{Introduction}%\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Language is the foundation on which communication rests allowing us to share ideas, and interact with each other. Cultures are built on this foundation, and you cannot understand a culture without the understanding of its language, which in turn is incubated and evolved by culture. Each culture is thus naturally best expressed using the language in which it evolved, which encodes knowledge about a people, their traditions, wisdom, environment, and how they interact with the sum of the concepts that belong to their culture. This is true about every language, including African languages.

%Culture and language are intricately linked. You cannot understand a culture without first learning a language, in fact, language evolves in a culture. It is one of the vehicles through which culture is expressed and every culture is best expressed in the language in which it evolves. Language expresses culture in an organized fashion. It encodes knowledge about a people, their tradition, wisdom, environment and how they interact with these concepts. 

The linguistic features of African languages, the presence or absence of concepts in the lexicons, all unveil important and often unique information about African languages, African people, their reality, their mind, as well a perspective about the world in which we live. Concepts for which words do not exist in African languages for instance are often foreign to the culture and experience of speakers of those languages. In these scenarios, speakers borrow words from other languages to fill these gaps or to communicate with people with a different language. This explains why there are certain words that are almost never borrowed since they occur in every human language. Here, we find kinship terms, body parts, words for basic bodily functions and sense perception terms, words for natural phenomena (‘sky’, ‘stone’, ‘ground’). These words, otherwise called basic vocabulary: are good for almost everything in language, from investigating human cognition to establishing language families.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}{}
\centering
\begin{adjustbox}{width=7cm}
\renewcommand{\arraystretch}{1.2}
{
  \includegraphics[width=10cm,height=8cm]{african_languages.jpg}}
  \end{adjustbox}
  \caption{African Languages in this paper}
\label{fig:our_map}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In NLP, about 50 out of 7,000 language \cite{joshi-etal-2020-state} have adequate language resources in the formats required to exploit advances in the field - an indication that the current state-of-the-art for many tasks knows very little about language in general. To make matters worse, most of these 50 languages belong to similar language families and share similar linguistic typologies - a convenient sample that cannot be generalized. Furthermore, despite the drive for language diversity and recent inclusions of many \texttt{low-resource} African languages in NLP, little or no attention is given to the unique differences of these languages. This leads to using methods and  automatic evaluation metrics built for languages with different typologies being forced on African languages. Claims are made about progress but how can true progress be measured if unique differences are not known? 

Language diversity bears particular significance given the international recognition by the global community of 2019 as the international year for indigenous languages and 2022-2032 as the international decade for indigenous languages. However, the idea of diversity in NLP will remain a mirage if attention is not given to unique linguistic differences. The fact that there hasn't been much computational / linguistic research on African languages, shows that intuitively there are some features that we cannot understand or solve without this level of understanding. The important information that can be learned from paying attention to unique differences will be lost in the current approach to NLP. 

Rule-based / knowledge-driven and data-driven \cite{GUDIVADA2015203} approaches are the major approaches to developing NLP. Knowledge driven systems leverage on linguistic rules while data-driven systems use large amounts of data. In this paper, we show that neither rule based nor data driven approaches are currently possible for many African languages due to: \textbf{(A)} language policy that results in low literacy in African languages, few "African" linguists, or computational linguists, and subsequent low or non-existent linguistic research, and \textbf{(B)} language policy and implementation that does not provide the environment for the collection of big data for many African languages. We provide detailed description of these issues in section \ref{sec:f_engineering}. 

%often require documentation of important  n\note[mam]{two main ways to develop nlp systems: knwoledge-based and end to end deep learning. Problems with each. We discuss issues with these in Section xx and Section yy. For everything we say we provide support references, quantify, or say there is no record or reference to depend on... \textbf{Problem a.} not enough linguists, cl people, cs people, no previous research sufficiently, \textbf{For problem b.} lack of data due to no sufficient efforts until recently to collect data, these recent efforts carried out with outside support that is usually not sufficient, not enough qualified annotators, no sufficient policy to streamline data collection (nothing similar to EU for example, or U.S. gov organizations like DARPA). }

%\texttt{The fact that there hasn't been much computational research on african languages, shows that intutitvely there are some features thatw e do not understand or solve without this level of understanding. It takes knowledge of how these languages work and how current approaches to different NLP problems can be applied to African languages.} 

%\texttt{The other approach to developing thses systems is to use large bodies of data. i.e an end-to-end deep learning approach that exploits large amounts of labelled and unlabelled data to discover and learn the required knowledge automatically. Neither of these two approaches is possible when working with African langauges. }

In conclusion, we argue that diversity should not be limited to the inclusion of more languages but the inclusion of methods that cater to the varied and unique properties of diverse languages. In this paper, we thus present a comprehensive survey of the state-of African languages in NLP. We provide research covering about 100 African languages. We analyse this based on the data, language typology, and methodology. In \ref{fig:our_map} we show a map of the languages covered in the survey and where L1 speakers of these languages are located in Africa. We provide geopolitical motivations for the state of many African languages as it relates to NLP, some prevalent linguistic typology of African languages that can be leveraged on for NLP development and an overview of NLP work in Africa.


==> motivation.tex <==
\section{Motivation}\label{sec:motivation}
Language is the foundation on which communication rests allowing us to share ideas, and interact with each other. Cultures are built on this foundation, and you cannot understand a culture without the understanding of its language, which in turn is incubated and evolved by culture \cite{fourie1995introduction}. Each culture is thus naturally best expressed using the language in which it evolved, which encodes knowledge about a people, their traditions, wisdom, environment, and how they interact with the sum of the concepts that belong to their culture. 

The presence or absence of concepts in the lexicon of African languages, the linguistic features of African languages, among other linguistics characteristics, all therefore unveil important and often unique information about African languages, African people, their reality, their mind, as well a perspective about the world in which we live. Concepts for which words do not exist in African languages for instance are often foreign to the culture and experience of speakers of those languages and speakers borrow words in these scenarios. This explains why there are certain words that are almost never borrowed since they occur in every human language.

Afro-centric methods, evaluation metrics, and datasets for African languages are therefore crucial to diversity in NLP.  



==> resources.tex <==
\section{Resources}\label{sec:resources}


%In recent times, there has been an increase in data collection efforts across multiple domains. Most datasets are collected as part of an NLP task and are often made available under the creative commons license. This makes them freely available to facilitate NLP research. Majority of the datasets available are for MT tasks, although the monolingual portion of the data can be used for other tasks. 

%create a table with labelled data and table for unlabelled data. remove url and make dataset names hyperlinks, add citations for datasets that were created in a paper. 


%\hl{Remember to refer to the tables in Appendix. Also if you will create an anonymous GitHub, you can provide a link earlier on. Also, we should try to put more than one table in a given page in Appendix. This is can be done later tomorrow perhaps, but it's something we should do. i.e., we should not put a small table on a whole appendix page. Also, we should create meaningful and informative captions for the table such that a reader would understand a lot about the table even if they have not read the text (carefully). I like Table 8!}

%\begin{table*}[!ht]

%\centering
%\begin{adjustbox}{max width=\textwidth}
%\renewcommand{\arraystretch}{1.15}
%\begin{tabular}{p{3cm}p{3cm}p{3cm}p{3cm}p{3cm}} 
%\hline
%\thead{\textbf{Language}} & \thead{\textbf{Tone}}  &  \thead{\textbf{Tone Marked}} &  \thead{\textbf{Vowel Harmony}} &  \thead{\textbf{SVC}} \\
%\hline  \hline
%Afar & None & None & &  \\
%Afrikaans & None & None &&\\
%Afan / oromo  & Yes & No & Yes & \\
%Akan & Yes & No & Yes & \\
%Twi & Yes & No & Yes & \\
%Akoose & Yes & Yes & Yes & \\
%Amazigh / Kabyle / Tamazight & No & No &&\\
%Amharic & No & No  &&\\
%Bambara /Bamanankan & Yes & no & yes &\\
%Bassa & yes & yes &&\\
%Bemba & yes & yes &&\\

%Coptic & No & No && \\
%Dagaare &Yes &No & Yes &Yes \\
%Dagbani&Yes &No & &\\
%Dangme &Yes &No & &\\
%Dendi
%Dinka & Yes & Yes &&\\
%Edo & Yes & Yes &&\\
%Efik & Yes & Yes &&\\
%Esan & Yes & No && \\
%Ewe & Yes & && \\
%Farafare Yes & No & Yes & \\
%Fula /Fulfude & No & No &  & \\
%Ga & Yes & No & Yes & \\
%Hausa & Yes & No & & \\
%Igbo & Yes & Yes & Yes & \\
%Igala & Yes & Yes & Yes & \\
%Isixhosa & Yes & No & & \\
%Isizulu & Yes & No & & \\
%Jula - Côte d’Ivoire \\
%Kabiye & Yes & Yes & Yes & \\
%Kamba & No & No && \\
%Kanuri & Yes & Yes & Yes & \\
%Kaonde &&&&\\
%Karaboro &&&&\\
%Kikuyu & Yes & No & Yes & \\
%Kirundi / Rundi &&&&\\
%Kissi & Yes & No && \\
%Kiswahili & No & No && \\
%Kituba / Kiluba  & No & No && \\
%Kongo & Yes & Yes ** & & \\
%Kpelle & Yes & Yes & & \\
%Kwangali &&&&\\
%Limba & No & No && \\
%Lukpa &&&&\\

%Lunda &&&&\\
%Luo & Yes & No && \\
%Malagasy & No & No && \\
%Mbukushu &&&&\\
%Medumba & Yes & Yes && \\
%Mende & Yes& No&& \\
%Mampruli &&&& \\
%Ndonga & No & NO &&\\
%Northern Sotho & No & NO &&\\
%Pular & No & NO &&\\
%Sango &Yes & Yes &&\\
%Setswana &Yes & No &&\\
%Sesotho  &Yes & No &Yes&\\
% & No & NO &&\\
%Shona &Yes & No &Yes&\\
%Swazi / Swati &Yes & No &&\\
%Somali &Yes & No &&\\
%Tachelhit - Morocco
%Tamajaq &&&&\\
%Themne &Yes & &&\\
%Tigrigna & No & NO &&\\
%Tiv & Yes & NO &&\\

%Tshivenda - South Africa

%Tumbuka - Malawi
%Urhobo - Nigeria
%Wolaytta - Ethiopia
%Wolof - Senegal
%Yemba / Dschang - Cameroon
%Yoruba & Yes & Yes & Yes & Yes \\
 %\end{tabular}
% \end{adjustbox}
 %\caption{List of available model resources}\label{tab:resources}
 %\end{table*}

%Add the language families


